Searching in the Forest for Local Bayesian Optimization

Because of its sample efficiency, Bayesian optimization (BO) has become a popular approach dealing with expensive black-box optimization problems, such as hyperparameter optimization (HPO). Recent empirical experiments showed that the loss landscapes of HPO problems tend to be more benign than previously assumed, i.e. in the best case uni-modal and convex, such that a BO framework could be more efficient if it can focus on those promising local regions. In this paper, we propose BOinG, a two-stage approach that is tailored toward mid-sized configuration spaces, as one encounters in many HPO problems. In the first stage, we build a scalable global surrogate model with a random forest to describe the overall landscape structure. Further, we choose a promising subregion via a bottom-up approach on the upper-level tree structure. In the second stage, a local model in this subregion is utilized to suggest the point to be evaluated next. Empirical experiments show that BOinG is able to exploit the structure of typical HPO problems and performs particularly well on mid-sized problems from synthetic functions and HPO.

==> Searching in the Forest for Local Bayesian Optimization/nomclat.tex <==
% Everything supposed to be used in equation mode?
% use in preamble: \input{macros_DAC.tex}

% Necessary packages for definitions
\usepackage{amsmath}
\usepackage{mathtools}  % for :=
\usepackage{amsfonts} 

\newcommand{\code}[1]{\small{\texttt{#1}}} 

%beginmacros

%--------- General Math Notation
\DeclareMathOperator*{\E}{\mathbb{E}}           % Expectation as a math operator
\DeclareMathOperator*{\expectation}{\mathbb{E}} % Expectation as a math operator
\renewcommand{\vec}[1]{\mathbf{#1}}             % Bold emphasis for vectors
\DeclareMathOperator*{\argmin}{arg\,min}        % Argmin
\DeclareMathOperator*{\argmax}{arg\,max}        % Argmax
\newcommand{\natnums}{{\mathbb{N}}}              % Notation for set of natural numbers
\newcommand{\realnums}{{\mathbb R}}             % Notation for set of real numbers
\newcommand{\extset}[2]{\{#1 \; | \; #2\}}      % Set of a given b. Renders {{a | b}}.    
\newcommand{\ddfrac}[2]{\frac{\displaystyle #1}{\displaystyle #2}}    % Double Display Fraction, forces large displays for everything in numerator and denominator

\newcommand{\diff}{\mathop{}\!\mathrm{d}}       % ???????
\newcommand{\transpose}[0]{{\textrm{\tiny{\sf{T}}}}} % Transpose T. Usage: $A^\transpose$
\newcommand{\norm}{{\mathcal{N}}}               % Normal distribution
\newcommand{\normaldist}{{\mathcal{N}}}         % Normal distribution
\newcommand{\iter}[2][\bocount]{{#2}^{(#1)}}    % Iteration specific instance of variable/function/anything

%-- Stochastic
\newcommand{\pdf}{\phi}                         % Standard Normal PDF
\newcommand{\cdf}{\Phi}                         % Standard Normal CDF
\newcommand{\mean}{\mu}                         % Mean
\newcommand{\stddev}{\sigma}                    % Standard Deviation
\newcommand{\variance}{\sigma^2}                % Variance
\newcommand{\noise}{\nu}                        % Noise
\newcommand{\given}[1][]{\:#1\vert\:}           % Conditional Probability "Given That" Relation, source: https://tex.stackexchange.com/a/141685/205886
\newcommand{\prob}[0]{p}                        % Probability p
\newcommand{\Prob}[0]{P}                        % Probability distribution P


%------- Notation for Configuration(s)

\newcommand{\confspace}[0]{\pmb{\Lambda}}       % Configuration space of parameters
\newcommand{\conf}[0]{\pmb{\lambda}}            % Configuration of parameters
%\newcommand{\bx}[0]{\conf}                     % Configuration of parameters
\newcommand{\hyperparam}{\lambda}               % Single hyperparameter of configuration
\newcommand{\hyperparami}[1][i]{{\hyperparam}_{#1}}   % Single hyperparameter within a hyperparameter configuration
\newcommand{\confinc}[0]{\pmb{\hat{\lambda}}}   % Incumbent configuration
%\newcommand{\confI}[1]{{\conf}^{(#1)}}      % Configuration corresponding to a given iteration -- better use \iter!
\newcommand{\confdef}[0]{{\conf}_{\text{def}}}  % Default configuration
\newcommand{\incumbent}[1][\bocount]{\iter[#1]{\confinc}}   % Incumbent configuration
\newcommand{\confincfin}{\incumbent[\bobudget]} % Final incumbent configuration (at end of run)
\newcommand{\confopt}[0]{{\conf}^*}             % Optimal configuration


%------- Notation for Cost, Risk, Loss, Performance Metric or Objective Functions

\newcommand{\loss}[0]{\mathcal{L}}              % Loss
\newcommand{\risk}{\mathcal{R}}                 % Risk
\newcommand{\riskemp}{\mathcal{R}_{\text{emp}}} % Empirical risk
\newcommand{\cost}[0]{c}                        % Cost
\newcommand{\costi}[1]{c^{(#1)}}                % Cost of instance/identifier
\newcommand{\objF}{F}                           % Family of objective functions
\newcommand{\func}[0]{f}                        % Function
\newcommand{\perfdomain}[0]{\mathbb{R}}         % Performance domain


%------- Notation for Algorithms
\newcommand{\algo}[0]{A}                        % One algorithm
\newcommand{\algos}[0]{\mathbf{A}}              % Set of algorithms    


\newcommand{\feat}[0]{\x_{\text{meta}}}                 % Meta features
\newcommand{\feats}[0]{\mathcal{X}_{\text{meta}}}       % Set of meta features


%------- Notation for Machine Learning
\newcommand{\dset}[0]{\mathcal{D}}                          % Dataset (instance)
\newcommand{\dsetmeta}[0]{\dset_{\text{meta}}}              % Dataset: meta
\newcommand{\dsettrain}[0]{\dset_{\text{train}}}            % Dataset: train
\newcommand{\dsetval}[0]{\dset_{\text{val}}}                % Dataset: val
\newcommand{\dsettest}[0]{\dset_{\text{test}}}              % Dataset: test
\newcommand{\x}[0]{\mathbf{x}}                              % Input vector x
\newcommand{\y}[0]{y}                                       % Output y
\newcommand{\xI}[1]{\mathbf{x}^{(#1)}}                      % i-th component of input
\newcommand{\yI}[1]{y^{(#1)}}                               % i-th component of output
\newcommand{\fx}{f(\mathbf{x})}                             % f(x), continuous prediction function
\newcommand{\Hspace}{\mathcal{H}}                           % hypothesis space where f is from
\newcommand{\fh}{\hat{f}}                                   % f hat, estimated prediction function


%------- Notation for Deep Learning
\newcommand{\weights}[0]{\theta}                            % Weights of neural network
\newcommand{\metaweights}[0]{\phi}                          % Weights of a meta-network


%------- Notation for AutoML
\newcommand{\portfolio}[0]{\mathbf{P}}                      % Portfolio
\newcommand{\schedule}[0]{\mathcal{S}}                      % Schedule
\newcommand{\hist}[0]{\dset_{\text{hist}}}                  % History


%------- Notation for Bayesian Optimization
%-- Components
\newcommand{\GP}{\mathcal{G}}                   % Gaussian Process
\newcommand{\kernel}{\kappa}                    % Kernel
\newcommand{\acq}{u}                            % Acquisition Function
\newcommand{\constraintg}{g}                    % Constraint function
\newcommand{\surro}[0]{\hat{\cost}}             % Surrogate model

%-- Loop
\newcommand{\bocount}{t}                        % BO loop counter
\newcommand{\bobudget}{T}                       % BO loop counter max, the counter runs from 1 to this value
\newcommand{\obs}[1][\conf]{\cost({#1})}        % BO loop observation
\newcommand{\obsspace}{\mathcal{Y}}             % BO loop observation space
\newcommand{\bonextobs}{\obs[\iter{\conf}]}     % BO loop next observation
\newcommand{\bonextsample}{\iter{\conf}}        % BO loop next selected sample

%-- Dataset
\newcommand{\dsetHPOdef}{{\langle \bonextsample,\,\bonextobs \rangle}_{\bocount=1}^{\bobudget}}     % Observed cost for selected configurations during BO run


%------- Notation for Reinforcement Learning
%-- Markov Decision Process with Components
\newcommand{\MDP}[0]{\mathcal{M}}                       % MDP (Markov Decision Process)
\newcommand{\statespace}[0]{\mathcal{S}}                % State space
\newcommand{\state}[0]{s}                               % State
\newcommand{\statet}[1][t]{\state_{#1}}                 % State at time t
\newcommand{\actionspace}[0]{\mathcal{A}}               % Action space
\newcommand{\action}[0]{a}                              % Action
\newcommand{\transdomain}[0]{\mathcal{T}}               % Transition domain (probability distribution of algorithm state transitions)
\newcommand{\trans}[0]{t}                               % Transition
\newcommand{\rewards}[0]{\mathcal{R}}                   % Reward function
\newcommand{\reward}[0]{r}                              % Reward

\newcommand{\policies}[0]{\mathbf{\Pi}}                 % Policies
\newcommand{\policy}[0]{\pi}                            % Policy
\newcommand{\policyopt}[0]{{\policy}^*}                 % Optimal policy

\newcommand{\discount}[0]{\gamma}                       % Discount rate
\newcommand{\valueS}[0]{\mathcal{V}}                    % State value function
\newcommand{\valueSip}[1][\inst]{\valueS^{\policy}_{#1}} % State value function under policy pi and instance i
\newcommand{\Qfunc}[0]{\mathcal{Q}}                     % State action value function (Q)
\newcommand{\Qfuncip}[1][\inst]{\Qfunc^{\policy}_{#1}}  % State action value function (Q) under policy pi and instance i

\newcommand{\egreedy}[0]{$\epsilon$-greedy}             % $\egreedy$ 

\newcommand{\trajectory}{\tau}                          % Trajectory
\newcommand{\episode}[0]{\mathcal{E}}                  % Episode
\newcommand{\expreturn}[0]{G}                           % Expected return
\newcommand{\cutoff}[0]{\kappa}                         % Cutoff kappa


%-- Dynamic Algorithm Configuration (DAC)
\newcommand{\inst}[0]{i}                    % One instance
\newcommand{\insts}[0]{\mathcal{I}}         % Set of instances
\newcommand{\insti}[1]{i^{(#1)}}            % Numbered instance. Usage: $\insti{3}$ for 3rd instance.

\newcommand{\cMDP}[0]{\MDP_\insts}                      % cMDP (contextual MDP)
\newcommand{\cMDPdef}[0]{\cMDP \coloneqq \{\MDPi\}_{\inst \sim \insts}} % cMDP: Definition as set of MDPs per instance
\newcommand{\MDPi}[0]{\MDP_\inst}                       % MDP of one instance
\newcommand{\MDPidef}[0]{\MDPi \coloneqq (\statespace, \actionspace, \transdomaini, \rewardsi)}  % MDP: Definition as tuple for one instance

\newcommand{\transdomaini}[0]{\transdomain_\inst}       % Transitions (instance-specific)
\newcommand{\rewardsi}[0]{\rewards_\inst}               % Rewards (instance-specific)    
\newcommand{\curric}[0]{\mathbf{d}}                     % Curriculum
\newcommand{\contexti}[1][i]{c_{#1}}                    % Context of instance i

\newcommand{\configspaceDAC}[0]{\Theta}                 % Configuration space
\newcommand{\configDAC}[0]{\theta}                      % Configuration
\newcommand{\hyperparamset}{H}                          % Hyperparameter set
\newcommand{\hyperparamname}[0]{h}                      % Name of hyper-/configuration parameter

%endmacros


% Regret
% Return
